A mean-field analysis of two-player zero-sum games

Finding Nash equilibria in two-player zero-sum continuous games is a central problem in machine learning, e.g. for training both GANs and robust models. The existence of pure Nash equilibria requires strong conditions which are not typically met in practice. Mixed Nash equilibria exist in greater generality and may be found using mirror descent. Yet this approach does not scale to high dimensions. To address this limitation, we parametrize mixed strategies as mixtures of particles, whose positions and weights are updated using gradient descent-ascent. We study this dynamics as an interacting gradient flow over measure spaces endowed with the Wasserstein-Fisher-Rao metric. We establish global convergence to an approximate equilibrium for the related Langevin gradient-ascent dynamic. We prove a law of large numbers that relates particle dynamics to mean-field dynamics. Our method identifies mixed equilibria in high dimensions and is demonstrably effective for training mixtures of GANs.

==> app_mckean.tex <==
\section{Exponential convergence of the entropy-regularized dynamics on toruses using McKean-Vlasov results} \label{sec:mckean}
\grant{This section needs a bit of housekeeping... let's try to state the main result, i.e., the contraction results at the beginning... we should discuss if it's worth including these results at all}
We will mostly use the theory developed by \citet{eberlequantitative2019}. They provide two results of convergence of McKean-Vlasov processes (their Theorems 2.3 and 2.4). They deal with McKean-Vlasov processes $Z$ on $\mathbb{R}^d$ of the following form:
\begin{align}
    \begin{split} \label{eq:mckean_vlasov_eberle}
        dZ_t &= b(Z_t) dt + \tau \int v(Z_t,z) d\mu_t(z) dt + dB_t, \\
        Z_0 &\sim \mu_0, \\
        \mu_t &= \text{Law}(Z_t)
    \end{split}
\end{align}
When we speak of solutions of SDEs we refer to strong solutions unless otherwise specified. We can recast the ERIWGF \eqref{eq:entropic_interacting_flow} as a McKean-Vlasov process for $Z_t = (X_t,Y_t)$ of the following form:
\begin{align}
    \begin{split} \label{eq:our_mckean_vlasov}
        d(X_t,Y_t) &= \int_{\mathbb{R}^{n_x} \times \mathbb{R}^{n_y}} \left( -\nabla_x \tilde{\ell}(X_t,y), \nabla_y \tilde{\ell}(x,Y_t) \right) d\mu_t(x,y) dt + \sqrt{2 \beta^{-1}}dB_t, \\
        (X_0,Y_0) &\sim \mu_0, \\
        \mu_t &= \text{Law}((X_t,Y_t))
    \end{split}
\end{align}
More precisely, if we take $\mu_0 = \mu_{x,0} \times \mu_{y,0}$, the marginals of the law of $(X_t, Y_t)$ are solutions to \eqref{eq:entropic_interacting_flow}.
\eqref{eq:our_mckean_vlasov} fits into \eqref{eq:mckean_vlasov_eberle} by first doing a change of variable on time $t'=2 \beta^{-1} t$, obtaining\footnote{I keep using $t$ instead of $t'$ for simplicity}
\begin{align}
    d(X_t,Y_t) &= \frac{\beta}{2} \int_{\mathbb{R}^{n_x} \times \mathbb{R}^{n_y}} \left( -\nabla_x \tilde{\ell}(X_t,\yy), \nabla_y \tilde{\ell}(\xx,Y_t) \right) d\mu_t(\xx,\yy) dt + dB_t
\end{align}
and then setting $Z_t = (X_t,Y_t)$, $b(\xx) \equiv 0$, $\tau = \beta / 2$, $v((\xx,\yy),(\xx',\yy')) = \left( -\nabla_x \tilde{\ell}(\xx,\yy'), \nabla_y \tilde{\ell}(\xx',\yy) \right)$. 

We will focus on Theorem 2.3 from \citet{eberlequantitative2019}, which is proven in the pages 32, 33 and 34 of the arxiv version of the article. Theorem 2.3 relies on two assumptions:
\begin{enumerate}
    \item Generalized one-sided Lipschitz condition on $b$: There exists a continuous function $\kappa: (0,\infty) \rightarrow \mathbb{R}$ such that $\int_0^1 r \kappa(r)\ dr < \infty$ and $\limsup_{r \rightarrow \infty} \kappa(r) < 0$ and
    \begin{align}
        \langle \xx-\yy,b(\xx)-b(\yy) \rangle \leq \kappa(|\xx-\yy|)|\xx-\yy|^2
    \end{align}
    for all $\xx,\yy \in \mathbb{R}^d$, $\xx \neq \yy$.
    \item Lipschitz condition on $\nu$: There exists a constant $L \in (0,\infty)$ such that for all $\xx,\yy,\xx',\yy' \in \mathbb{R}^d$,
    \begin{align}
        |\nu(\xx,\xx')-\nu(\yy,\yy')| \leq L(|\xx-\yy|+|\xx'-\yy'|)
    \end{align}
\end{enumerate}
To state the conclusion of Theorem 2.3, let us define 
\begin{align}
    \rho_0(x,y) = f(|x-y|)
\end{align}
where $f:\mathbb{R}_+ \rightarrow \mathbb{R}_+$ is a non-decreasing concave continuous function such that $f(0) = 0$. Theorem 2.3 specifies a particular $f$ and in our argument we will use a different one. We define the Wasserstein distance
\begin{align}
    \mathcal{W}_{\rho_0}(\nu,\mu) := \inf_{\gamma \in C(\nu,\mu)} \int \rho_0(x,y) \ d\gamma(x,y)
\end{align}
Notice that under the appropriate conditions on $f$, $\mathcal{W}_{\rho_0}$ and
\begin{align}
    \mathcal{W}_1(\nu,\mu) := \inf_{\gamma \in C(\nu,\mu)} \int |x-y| \ d\gamma(x,y)
\end{align}
are equivalent.

The conclusion of Theorem 2.3 of \citet{eberlequantitative2019} is that there exist constants $c, K$ such that
\begin{align}
\begin{split} \label{eq:thm2.3}
\mathcal{W}_{\rho_0}(\nu_t,\mu_t) &\leq \text{exp}((|\tau|K-c)t) \ \mathcal{W}_{\rho_0}(\nu_0,\mu_0) \\
\mathcal{W}_1(\nu_t,\mu_t) &\leq 2 \ A \ \text{exp}((|\tau|K-c)t) \ \mathcal{W}_1(\nu_0,\mu_0)
\end{split}
\end{align}
where $\mu_t$ and $\nu_t$ are solutions of \eqref{eq:mckean_vlasov_eberle} initialized at $\mu_0, \nu_0$ respectively.
The second equation of \eqref{eq:thm2.3} follows from the first one by the equivalence of the distances. This implies that up to a certain value of $\tau$ ($\tau < c/K$), the solutions of \eqref{eq:mckean_vlasov_eberle} converge exponentially in $\mathcal{W}_1$ regardless of their initial measures. 

\textit{Why would we want to have a statement like the one provided by Theorem 2.3 of \citet{eberlequantitative2019}?}
%By Proposition 8 of \url{stationary_distribution.tex} we know there exists $\hat{\mu} = \hat{\mu}_x \times \hat{\mu}_y$ such that $\mu_t = \hat{\mu}, \ \forall t \geq 0$ is a solution of \eqref{eq:mckean_vlasov_eberle} (i.e. $\hat{\mu}$ is a stationary measure of the McKean-Vlasov process). 
By \autoref{thm:stationary_point}, we know that there exists a unique pair $\hmu_x, \hmu_y$ that is a stationary solution of \eqref{eq:entropic_interacting_flow}, and we are interested in finding it because we know it is an $\epsilon$-Nash equilibrium by \autoref{thm:epsilon_thm} and \ref{thm:stationary_point}. If we initialize \eqref{eq:our_mckean_vlasov} with a random variable of law $\hmu_x \times \hmu_y$, then the law of the process is $\hmu_x \times \hmu_y$ at all times

Applying \eqref{eq:thm2.3} for $\mu_t=\hmu_x \times \hmu_y$ we obtain 
\begin{align}
    \mathcal{W}_1(\nu_t,\hat{\mu}_x) = \mathcal{W}_1(\nu_t,\mu_t) \leq 2 \ A \ \text{exp}((|\tau|K-c)t) \ \mathcal{W}_1(\nu_0,\mu_0) = 2 \ A \ \text{exp}((|\tau|K-c)t) \ \mathcal{W}_1(\nu_0,\hat{\mu})
\end{align}
for any initial $\nu_0$. This gives a rate of convergence to the stationary measure, which is what we seek for.

\textit{Why is Theorem 2.3 of \citet{eberlequantitative2019} not suitable in our case?}
We are considering a McKean-Vlasov processes in compact manifolds without boundary (in particular the $d$-dimensional torus for simplicity, with $d = d_x + d_y$). We can consider the corresponding McKean-Vlasov process in $\mathbb{R}^d$. Notice that in this case $b \equiv 0$ and hence the assumption $\limsup_{r \rightarrow \infty} \kappa(r) < 0$ fails because the best $\kappa$ we can choose is $\kappa \equiv 0$.

\carles{Keep looking at this.}
\subsection{The modifications on the proof of Theorem 2.3 of \citet{eberlequantitative2019}}
\carles{State theorem.}
We will only use the Lipschitzness assumption on $\nu$.
Similarly to \citet{eberlequantitative2019} but with a slightly different notation, we define 
$\tilde{Z}_t = X_t - Y_t$ and $\tilde{r}_t = \|X_t - Y_t\|_2$, where $\|\cdot\|_2$ is the $l^2$ norm.

Let us we define $\pi: \mathbb{R}^n \rightarrow [0,1)^n$ as $(x_1,...,x_n) \mapsto (y_1,...,y_n)$ such that $\forall i \in [1:n], \ y_i \in [0,1)$ and $y_i - x_i \in \mathbb{Z}$. The $N$-dimensional torus $\mathbb{T}^n$ is then defined as the topological space given by the set $[0,1)^n$ and the final topology induced by $\pi$ (i.e. the finest topology in $[0,1)^n$ that makes $\pi$ continuous). We consider $\mathbb{T}^n$ as a Riemannian manifold with the differentiable and metric structure inherited from $\mathbb{R}^n$ through $\pi$. 

Notice that $\pi$ allows us to map any Borel measure $\mu$ on $\mathbb{R}^n$ to its pushforward measure $\pi_{*} \mu$, defined as $\pi_{*} \mu (B) = \mu(\pi^{-1}(B))$ for all Borel-measurable subsets $B$ of $\mathbb{R}^n$. $\pi$ also allows us to map any $\mathbb{R}^n$-valued random variable (or rather, $\mathbb{R}^n$-valued random element) $X$ into a $\mathbb{T}^n$-valued random element $\pi(X)$. Similarly, we can map a $C([0,T],\mathbb{R}^n)$-valued random element $X$ into a $C([0,T],\mathbb{T}^n)$-valued random element $\hat{\pi}(X)$ defined as 
\begin{equation}\label{def:hat_pi}\hat{\pi}(X)(t) = \pi(X(t)). \end{equation} 

We also define the map $\pi': [0,1)^d \rightarrow [0,1/2)^d$ component-wise, i.e. for $k \in \{1,...,d\}$ the $k$-th component of $\pi'(x)$ is defined in terms of the $k$-th component of $x$ as
\begin{align}
    \pi'_k(x) := \begin{cases}
    x_k & \text{if } x_k \in [0,1/2) \\
    1-x_k & \text{if } x_k \in [1/2,1)
    \end{cases}
\end{align}
We define $Z_t=(\pi' \circ \pi)(X_t-Y_t)$ and $r_t = \|Z_t\|_2$, where $d_\mathbb{T}$ is the distance on the torus induced by the $l_2$ distance in $\mathbb{R}^d$. 

Using the same coupling for $X_t, Y_t$, notice that the following equation from \citet{eberlequantitative2019}
\begin{align}
    d\tilde{Z}_t = (b^{\mu_0}(t,X_t) - b^{\nu_0}(t,Y_t)) dt + 2 \text{rc}(U_t)e_t dW_t 
\end{align}
holds in our case for $\tilde{Z}_t$, where
\begin{align}
\begin{split}
    b^{\mu_0}(t,X_t) &= \tau \int v(X_t,\xx) d\mu_t(\xx) dt, \\
    b^{\nu_0}(t,Y_t) &= \tau \int v(Y_t,\yy) d\mu_t(\yy) dt.
\end{split}
\end{align}
The corresponding equation for $Z_t$ in our case is
\begin{align}
    dZ_t = s(Z_t)\odot(b^{\mu_0}(t,X_t) - b^{\nu_0}(t,Y_t)) dt + 2 \text{rc}(U_t) s(Z_t)\odot e_t dW_t. 
\end{align}
where $s(\cdot)$ are vectors in $\mathbb{R}^d$ and $\odot$ is the component-wise vector multiplication. Specifically, the component $k \in \{1,...,d\}$ of $s(\mathbf{z})$ is defined as
\begin{equation}
    s_k(z) := \begin{cases}
    1 & \text{if } z_k \in [0,1/2) \\
    -1 & \text{if } z_k \in [1/2,1)
    \end{cases}
\end{equation}
The analog of (5.25) from \citet{eberlequantitative2019} holds in our case for $\tilde{r}_t$ in the following form
\begin{align}
    dr_t = \langle \tilde{e}_t, s(Z_t)\odot (b^{\mu_0}(t,X_t) - b^{\nu_0}(t,Y_t) )\rangle dt + 2 \text{rc}(U_t) dW_t
\end{align}

(5.29) and (5.30) from \citet{eberlequantitative2019} rewrite as:
\begin{align}
\begin{split}
\langle \tilde{e}_t, s(Z_t)\odot (b^{\mu_0}(t,X_t) - b^{\nu_0}(t,Y_t)) \rangle &= \langle \tilde{e}_t, s(Z_t)\odot (\tilde{b}^{\tilde{\mu}_0}(t,\tilde{X}_t) - \tilde{b}^{\tilde{\nu}_0}(t,\tilde{Y}_t)) \rangle \leq |\tau| L (r_t + \mathcal{W}_1(\tilde{\mu}_t,\tilde{\nu}_t)) \\ &\leq |\tau| L (r_t + \mathbb{E}[r_t]) 
\end{split}
\end{align}
%Suppose 
Let $f:[0,\infty) \rightarrow \mathbb{R}$ such that
\begin{align} \label{eq:f_def}
    c r + 2 f''(r) = 0, \ f(0)=0
\end{align}
Integrating the equation, we obtain
\begin{align}
\begin{split}
    f'(r) &= -\frac{c}{4}r^2 + k \\
    f(r) &= -\frac{c}{12}r^3 + kr
\end{split}
\end{align}
Let us set $k=\frac{c}{4}$ such that $f$ is increasing in $[0,1]$. Notice that $f$ is concave in $[0,1]$.
Also, for $r \in [0,1]$
\begin{align} \label{eq:derivative_bound}
    f'(r) \leq \frac{c}{4} 
\end{align}
Let us set
\begin{align} \label{eq:gamma_def}
\gamma := c - \frac{c}{2}|\tau|L > 0.
\end{align}
This imposes the constraint $|\tau|<2/L$.
%\begin{align}
%    \forall r \in [0,1], -2f''(r) - 2|\tau|L|f'(r)r \geq \epsilon f'(r) r \geq \gamma r
%\end{align}

Notice that
(5.31) rewrites as
\begin{align}
    \begin{split} \label{eq:development_5.31}
        d(e^{\gamma t} f(r_t)) &= e^{\gamma t} dM_t + e^{\gamma t} (\gamma f(r_t) + H_t) dt \leq e^{\gamma t} dM_t + e^{\gamma t} (\gamma r_t + H_t) dt \\ &\leq 
        e^{\gamma t} dM_t + e^{\gamma t} (\gamma r_t + |\tau| L (r_t + \mathbb{E}[r_t]) f'(r_t)) dt + 2 e^{\gamma t} f''(r_t) dt \\ &\leq e^{\gamma t} dM_t + e^{\gamma t} ((c - \frac{c}{2}|\tau|L)r_t + |\tau| L \frac{c}{4}(r_t + \mathbb{E}[r_t])) dt + 2 e^{\gamma t} f''(r_t) dt \\ &= e^{\gamma t} dM_t + e^{\gamma t} |\tau| L \frac{c}{4}(\mathbb{E}[r_t] - r_t)
    \end{split}
\end{align}
In the second inequality we use the definition of $\gamma$ in equation \eqref{eq:gamma_def} and the bound on $f'$ of equation \eqref{eq:derivative_bound}. In the last equality we cancel terms, using \eqref{eq:f_def}. 

As in \citet{eberlequantitative2019}, \eqref{eq:development_5.31} yields 
\begin{align}
    \mathbb{E}[e^{\gamma t} f(r_t) - f(r_0)] \leq 0,
\end{align}
which implies
\begin{align}
    \mathcal{W}_{\rho_0}(\mu_t,\nu_t) \leq \mathbb{E}[\rho_0(X_t,Y_t)] = \mathbb{E}[f(d_{\mathbb{T}}(\pi(X_t),\pi(Y_t)))] = \mathbb{E}[f(r_t)] \leq \frac{\mathbb{E}[f(r_0)]}{e^{\gamma t}} = \frac{\mathcal{W}_{\rho_0}(\mu_0,\nu_0)}{e^{\gamma t}}.
\end{align}
The last equality follows from $\mathbb{E}[f(r_0)] = \mathcal{W}_{\rho_0}(\mu_0,\nu_0)$, which used in \citet{eberlequantitative2019} and is common in contraction results.

==> future_work_old.tex <==
\section{Conclusions and future work}

In this work we have explored non-convex-non-concave, high-dimensional 
games from the perspective of optimal transport. 
Similarly as with non-convex optimization over a high-dimensional space, expressing the problem in terms of the underlying measure provides important geometric benefits, at the expense of moving into non-Euclidean metric spaces over measures. 
Our main theoretical results establish approximate mean-field 
convergence under two important setups: Langevin Descent-Ascent 
and WFR Descent-Ascent. Our theory directly applies to challenging yet important setups such as GANs, bringing guarantees for sufficiently overparametrised generators and discriminators. 

Despite such positive convergence guarantees, our results 
are qualitative in nature, i.e. without rates.
%we do not currently have rates of convergence with respect to the number of particles nor time. 
In the entropic case, our analysis suffers from an unfavorable tradeoff between temperature and convergence of the associated McKean-Vlasov scheme; while the techniques of \citep{eberlequantitative2019} are very general, they don't leverage the structure of our problem setup, so it may be interesting to explore Log-Sobolev-type inequalities in this context instead \citep{Markowich99onthe}.  
In the WFR case, we are lacking a local convergence analysis that would explain the benefits of transport that we observe empirically, for instance leveraging sharpness Polyak-Łojasiewicz results such as those in \citep{chizat2019sparse} or \citep{sanjabi2018solving}.
 %along with establishing a CLT to quantify the scale of fluctuations. 
 Another important open question is to obtain Central Limit Theorems for the convergence of the particle dynamics to the mean field dynamics,
 in the Langevin, the Wasserstein-Fisher-Rao and the pure mirror descent cases. We expect to see the magnitude of the fluctuations to blow-up with dimension for mirror descent, as that would explain the poor performance of its associated particle dynamics. 
 For the Langevin and Wasserstein-Fisher-Rao cases, it is reasonable to expect a moderate growth of the fluctuations, in light of our numerical experiments. 
 Finally, in our GAN formulation, each generator is associated to a single particle in a high-dimensional product space of all network parameters. In that sense, we are currently not exploiting the exchangeablility of the neurons, as is done for instance in the single-hidden layer mean-field analyses \citep{mei2018mean, chizat2018global, rotskoff2018neural, sirignano2019mean}. A natural question is to understand to what extent our framework could be combined with specific choices of architecture, as recently studied in \citep{lei2019sgd}. 

% did not exploit the architectural aspects of GANs in our formulation, in which we treat the ensemble of parameters as a single strategy rather than as a mixture itself, as recently studied in \citep{lei2019sgd}. 
%  Better parametrisation of the generator mixture to scale up GAN experiments. Currently our generator architecture can be seen as having a wide final layer, with independent networks operating in parallel below. One could devise more efficient mixture strategies with better complexity that preserve the benefits of our framework. 
 

%\joan{add something about limitation of our GAN experiments.}
%Some of these aspects may be within reach as future steps. Specifically, we identify
%Future steps include
% (i) Obtaining Central Limit Theorems for the convergence of the particle dynamics to the mean field dynamics, and
 %in the Langevin, the Wasserstein-Fisher-Rao and the pure mirror descent cases. We expect to see the magnitude of the fluctuations to explode in time for pure mirror descent, as that would explain the poor performance of the particle dynamics. For the Langevin and Wasserstein-Fisher-Rao cases, it is reasonable to expect a controlled growth of the fluctuations. 
 %(ii) Establishing convergence for the WFR dynamics that does not require to make the transport term arbitrarily small in order to reach a given value for the NI error. %This could come in the form of a local convergence result, and the current argument could be used to reach a point where the local convergence assumptions are fulfilled. 
% (iii) Leverage overparametrisation in the GAN formulation to increase mixture size with reduced computational costs. 
 

% \samy{I find the future work long. maybe we should reduce it and mention just one/two directions. }
 
% \begin{itemize}
%     \item Obtaining central limit theorems and fluctuation results for the convergence of the particle dynamics to the mean field dynamics in the Langevin, the Wasserstein-Fisher-Rao and the pure mirror descent cases. We expect to see the magnitude of the fluctuations to explode in time for pure mirror descent, as that would explain the poor performance of the particle dynamics. For the Langevin and Wasserstein-Fisher-Rao cases, it is reasonable to expect a controlled growth of the fluctuations.
%     \item Obtaining a convergence result for the Wasserstein-Fisher-Rao dynamics that does not require to make the transport term arbitrarily small in order to reach a given value for the Nikaido-Isoda error. This could come in the form of a local convergence result, and the current argument could be used to reach a point where the local convergence assumptions are fulfilled. A more ambitious endeavor would be to devise an argument that captures the benefits of the transport term in the WFR dynamics instead of viewing it as a harmful perturbation to mirror descent.
%     \item Deriving convergence rates for the Langevin mean-field dynamics, beyond the $\beta < O(1/L)$ regime. Interesting results could be in analogy to the Holley-Stroock perturbation lemma and the Bakry-Emery theorem in the literature of potential Fokker-Planck equations (see Section 5 of \citet{Markowich99onthe} for an overview).
% \end{itemize}
